Sample Complexity for Non-Truthful Mechanisms

This paper considers the design of non-truthful mechanisms from samples. We identify a parameterized family of mechanisms with strategically simple winner-pays-bid, all-pay, and truthful payment formats. In general (not necessarily downward-closed) single-parameter feasibility environments we prove that the family has low representation and generalization error. Specifically, polynomially many bid samples suffice to identify and run a mechanism that is $\epsilon$-close in Bayes-Nash equilibrium revenue or welfare to that of the optimal truthful mechanism with high probability.

==> binningapp.tex <==
\section{Proof of \Cref{THM:WELARE}}
\label{app:approximation}

In this appendix, we derive a surrogate-ranking mechanism with near-optimal welfare or revenue, which proves the following theorem, restated for convenience:
\begin{numberedtheorem}{\ref{thm:welfare}}
There exists a surrogate-ranking with winner-pays-bid, all-pay, or
truthful payment semantics which attains a $(1-
O(\sqrt[3]{n/\num}))$-fraction of the optimal welfare in stationary equilibrium. With regular distributions, there exists such a mechanism which attains a $(1-
O(\sqrt[3]{n/\num}))$-fraction of the optimal revenue in stationary
equilibrium.
\end{numberedtheorem}

Before proving the main theorem, we observe that a less general result
follows from a theorem of \citet{HKM11}. In this paper, the authors
consider an allocation procedure which can be interpreted as a surrogate ranking
mechanism. They show that for agents whose values are
distributed on the interval $[0,1]$, their mechanism has an additive welfare loss of at most $n/(4\sqrt T)$. 
% Because we derive the
% welfare-optimal surrogate-ranking mechanism, we inherit this welfare
% guarantee. In particular, we have:
% \begin{corollary}[\citet{HKM11}]
% \label{cor:hkm}
% In any feasibility setting, if agents have value distributions on $[0,1]$, then in the symmetric equilibrium, the welfare-optimal surrogate-ranking mechanism loses at most an additive $n/(4\sqrt T)$ per stage with respect to the welfare of the optimal mechanism.
% \end{corollary}
%per-round loss or average loss per round.
We improve on this welfare guarantee in three ways. First, we derive a guarantee for arbitrary distributions, even those with unbounded support. Second, our bounds will be multiplicative. Finally, our bounds apply to revenue in addition to welfare.\footnote{With the additional assumption that virtual values are bounded below by $-\underline \phi$, the guarantee of \citet{HKM11} applies to revenue as well, with an additional factor of $1+\underline \phi$ applied to the loss.}


\input{rankvpriceapp}


We can further generalize Lemma~\ref{lem:rankvprice} by comparing
distributions over pricing algorithms with the analogous distributions
over top-$k$ algorithms. As long as prices avoid the extremes of the
distribution, ranking performs well with respect to pricing.

\begin{lemma}
\label{lem:distprice}
Consider a distribution over $k/\num$-price posting algorithms for $\num$ agents, where the highest price is at quantile $\underline k/\num$ and the lowest price is at quantile $\overline k/\num$. The same distribution over corresponding top-$k$-of-$\num$ algorithms attains a $(1-O({\underline k}^{-1/2}))$-fraction of the welfare of the distribution over price-posting algorithms. If values are regularly distributed, then the distribution over top-$k$-of-$\num$ algorithms attains a $(1-O(\min(\underline k,T-\overline k)^{-1/2}))$-fraction of the price-posting revenue as well.
\end{lemma}

\begin{proof}
Lemma~\ref{lem:rankvprice} implies that for each price in the distribution of the price-posting algorithm, there is a top-$k$-of-$\num$ algorithm which approximates it and which appears with the same probability. The approximation ratio of a distribution over pairwise approximations is at least the approximation from the worst pair. 
%Note that the approximations from Lemma~\ref{lem:rankvprice} are symmetric about $1/2$, and are worst for very low and very high $k$. It follows that the approximation ratio is driven by the $\underline k/\num$- and $\overline k/\num$-price posting algorithm.
\end{proof}

\subsection{Binning Versus Ranking}

Lemma~\ref{lem:distprice} shows that in simple settings, ranking can
discriminate with almost as much
accuracy as pricing. We now extend this idea to the setting of general mechanism design with runtime samples. We compare the allocation rule of a surrogate ranking mechanism (i.e. a \emph{surrogate ranking algorithm}) with a
{\em surrogate binning algorithm}, which assigns agents a surrogate value by dividing quantile space into coarse ``bins'' of uniform probability and associating each bin with a surrogate value. We formally define this algorithm as follows.

\begin{definition}
	\label{def:binning}
	Given a set of $\num$ surrogate values $\Psi$ with
	$\psi^1\geq\ldots\geq\psi^{\num}$, the \emph{binning} selection rule for $\Psi$ maps each input quantile $q$ to $\psi^j$ for the $j$ for which $q\in [(j-1)/\num,j/\num]$.
\end{definition}

\begin{definition}
For surrogate values
$\{\Psi_i\}_{i=1}^n$, and binning surrogate selection rules
$\{\sigma_i\}_{i=1}^n$, the \emph{surrogate binning algorithm} is
given by computing $\mathbf{\tilde x}({\mathbf \quant})=
\argmax_{\mathbf x}\sum_{i}x_i\sigma_i(\quant_i)
$.
\end{definition}

Any allocation rule can be viewed by agents as a distribution over posted prices. We note several properties of surrogate-binning algorithms which make this distribution easy to analyze. First, note that because quantiles are uniform for each agent, the distribution of surrogate values input to the allocation algorithm is also uniform. Second, because surrogate-binning mechanisms treat agents coarsely based on the bin into which their quantile falls, and because bins are distributed evenly in quantile space, it follows that for surrogate-binning mechanisms, the distribution over posted prices can actually be viewed as a distribution over $k/\num$-quantile price posting algorithms. 

Meanwhile, a standard fact from the study of position auctions is that any rank-based position auction can be represented as a convex combination of $k$-unit auctions. Since the allocation rule agents face in a surrogate-ranking mechanism is identical to that of a rank-based position auction, a similar analysis applies. We summarize the above discussion with the following lemma:
%
%
%
%\label{sec:bvr}
%%\begin{definition}
%%Given a monotone stage allocation algorithm $\mathbf{\hat x}$ and lists of surrogate values $\psi_i^1\geq \psi_i^2\geq\ldots\geq \psi_i^T$ for each distribution $i$, the \emph{surrogate-binning mechanism} for $\mathbf{\hat x}$ and $\{\psi_i^j\}$ assigns all agents  from distribution $i$ with quantile $q_i^t\in [\tfrac{j-1}{T},\tfrac{j}{T}]$ surrogate value $\psi_i^j$. It then runs $\mathcal A$ on each stage's profile of surrogate values, and allocates agents accordingly.
%%\end{definition}
%
%We now show that surrogate-binning algorithms can be well-approximated by ranking algorithms. The
%allocation rules of binning algorithms appear to agents as
%piecewise constant functions. Hence, each population $i$ sees a
%distribution over $k/T$-price posting algorithms. Moreover, in the
%batched population environment, we may rank rather than price,
%just as in Lemma~\ref{lem:distprice}. By ranking each
%agent and treating the agent with rank $j$ as if they were in the
%$j$th bin, we produce a surrogate-ranking
%algorithm. Lemma~\ref{lem:distprice} implies that this algorithm
%performs almost as well as the binning algorithm, provided that the
%prices from the binning algorithm do not come from extreme quantiles.
%
%
%\begin{theorem}
%\label{thm:bvr}
%For monotone stage algorithm $\mathbf{\hat x}$ and surrogate values
%$\psi_i^1\geq \psi_i^2\geq\ldots\geq \psi_i^T$ with
%$\psi_i^1=\psi_i^2=\ldots=\psi_i^{\underline k}$ and
%$\psi_i^{\overline k}=\psi_i^{\overline k+1}=\ldots=\psi_i^T$ for each
%population $i$, the surrogate ranking algorithm attains a
%$\rho(\min(\underline k, T-\overline k),T)$-fraction of the welfare of
%the binning algorithm. If distributions are regular, then the
%surrogate ranking algorithm attains a $\eta(\min(\underline k,
%T-\overline k),T)$-fraction of the binning algorithm's virtual
%surplus.
%\end{theorem}
%
%To derive Theorem~\ref{thm:bvr}, note that by Lemmas~\ref{lem:uniformity} and~\ref{lem:characteristics}, the surrogate-binning algorithm allocates agents according to its characteristic weights. Moreover, we already showed in Section~\ref{sec:eq} that surrogate-ranking algorithms also allocate agents according to characteristic weights. Thus if the two algorithms use the same surrogate values, these characteristic weights will be the same. Next, note that the surrogate-binning and surrogate-ranking algorithms appear to agents as distributions over pricing and top-$k$ algorithms, respectively, with the distributions determined by marginal characteristic weights. Formally:
%
\begin{lemma}
\label{lem:bin}
Any surrogate-binning (resp. surrogate-ranking) algorithm with surrogate values $\{\psi_i^j\}^{j=1,\ldots,T}_{i=1,\ldots,n}$ appears to agents in each distribution $i$ as a distribution over price-posting (resp. top-$k$) algorithms. The probability of offering the price with quantile $\tfrac{j}{T}$ (resp. of allocating $j$ units) is given by $w_i^{j}-w_i^{j+1}$, where $w_i^0 = 1$, $w_i^{T+1}=0$, and $w_i^j$ is the characteristic weight for $\psi_i^j$ for $j=1,\ldots, T$.
\end{lemma}

Notice that if
$\psi_i^1=\ldots=\psi_i^{\underline k}$ for some positive integer $\underline k$, the binning algorithm's
allocation rule on the first $\underline k$ intervals of distribution
$i$'s quantile space will be constant. If $\psi_i^{\overline k}=\ldots=\psi_i^T$ for some positive integer $\overline k$, then the allocation rule on the last $T-\overline k$ intervals will be constant. In terms of distribution $i$'s
randomization over posted pricings, the highest nontrivial price
offered has quantile $\underline k/n$, and the lowest has quantile
$\overline k/n$. These extremal quantiles drive the approximation
guarantees relating pricing to ranking and, thus, good approximation
bounds can be obtained via Lemma~\ref{lem:distprice} if there is not
much loss in restricting to binning algorithms that price at moderate
quantiles. Consequently, we obtain the following theorem:

\begin{theorem}
\label{thm:bvr}
For surrogate values
$\psi_i^1\geq \psi_i^2\geq\ldots\geq \psi_i^T$ with
$\psi_i^1=\psi_i^2=\ldots=\psi_i^{\underline k}$ and
$\psi_i^{\overline k}=\psi_i^{\overline k+1}=\ldots=\psi_i^T$ for each
population $i$, the surrogate ranking algorithm attains a
$(1-O(\underline k^{-1/2}))$-fraction of the welfare of
the binning algorithm. If distributions are regular, then the
surrogate ranking algorithm attains a $(1-O(\min(\underline k,T-\overline k)^{-1/2}))$-fraction of the binning algorithm's virtual
surplus.
\end{theorem}

\begin{proof}
First note that to agent $i$, the distribution of surrogate values among agents from other agents is identical between binning and ranking - each surrogate value appears with probability $1/T$, independently across distributions. It follows that each surrogate value has the same characteristic weight in both mechanisms. Therefore the distribution of prices from the surrogate-binning mechanism matches the distribution over top-$k$ mechanisms from the surrogate-ranking mechanism.
Note that these distributions might involve prices and $k$ for which 0 or $T$ agents get allocated. For purposes of approximation, these cases can be ignored, as the corresponding pricing and top-$k$ mechanisms perform identically. It follows that we may apply Lemma~\ref{lem:distprice}. If  $\psi_i^1=\ldots=\psi_i^{\underline k}$ and $\psi_i^{\overline k}=\ldots=\psi_i^T$, then we have that the most extreme nontrivial values of $k$ are $\underline k$ and $\overline k$. This yields the stated bound.
\end{proof}
%
%Finally, Theorem~\ref{thm:bvr} follows from applying
%Lemma~\ref{lem:distprice}. Notice that if
%$\psi_i^1=\ldots=\psi_i^{\underline k}$, the binning algorithm's
%allocation rule on the first $\underline k$ intervals of distribution
%$i$'s quantile space will be constant. In terms of distribution $i$'s
%randomization over posted pricings, the highest nontrivial price
%offered has quantile $\underline k/n$, and the lowest has quantile
%$\overline k/n$. These extremal quantiles drive the approximation
%guarantees relating pricing to ranking and, thus, good approximation
%bounds can be obtained via Lemma~\ref{lem:distprice} if there is not
%much loss in restricting to binning algorithms that price at moderate
%quantiles.
%
%
%%First note that to agent $i,t$, the distribution of surrogate values among agents from other distributions is identical between binning and ranking - each surrogate value appears with probability $1/T$, independently across distributions. It follows that each surrogate value has the same characteristic weight in both mechanisms. It follows from Lemmas~\ref{lem:bin} and~\ref{lem:rank} that the distribution of prices from the surrogate-binning mechanism matches the distribution over top-$k$ mechanisms from the surrogate-ranking mechanism.
%
%%As we have seen, the respective distributions over prices and top-$k$ mechanisms for binning and ranking are identical. Note that the above distributions might involve prices and $k$ for which 0 or $T$ agents get allocated. For purposes of approximation, these cases can be ignored, as the corresponding pricing and top-$k$ mechanisms perform identically. It follows that we may apply Lemma~\ref{lem:distprice}. If  $\psi_i^1=\ldots=\psi_i^{\underline k}$ and $\psi_i^{\overline k}=\ldots=\psi_i^T$, then we have that the most extreme nontrivial values of $k$ are $\underline k$ and $\overline k$. This yields the stated bound.

\subsection{Approximately Optimal Binning}

We now show how to construct an approximately welfare- or revenue-optimal binning algorithm with large first and last bin. Combined with
\Cref{thm:bvr}, this construction implies
Theorem~\ref{thm:welfare}. We will choose surrogate values via resampling. That is, we will map the $j$th surrogate of
agent $i$, which corresponds to an agent with quantile in $[\tfrac{j-1}{T},\tfrac{j}{T}]$ %, denoted
%%$F_i[\tfrac{j-1}{T},\tfrac{j}{T}]$,
 to a redrawn value from their value distribution conditioned to this interval.  Such resampling does not change the induced
allocation rule for any other agents, and replaces the allocation rule for agent $i$
on their $j$th quantile interval with its average.

This basic approach does not directly lead to the desired approximation
bound. For an example where this fails, note that for the top quantile interval, the allocation
probability at the very top of the interval may be much higher than its
average across the interval, while the highest values on the interval may
be much higher than the interval's average.  For example, if the value
and allocation rule are both $1$ for an $\epsilon$ measure and zero
otherwise, then the original welfare is $\epsilon$ and the welfare
from resampling is $\epsilon^2$.  A second issue is that we wish to be
able to apply \Cref{thm:bvr} to get a good approximation bound.
For example, we would get a $1-k^{-1/2}$ bound for welfare if the top $k$
 intervals have the same allocation probability.


To resolve both these issues, we will first modify the allocation rule to
treat agents with values in the top $k$ intervals as if they had the
highest value in the support of their distributions, and treat agents with values in the bottom $k$ intervals as if they had the lowest value in the support of their distributions, for some given positive integer $k$.  The quantiles of
the remaining agents will be rescaled. Conditioned on the
values not being in the top or bottom $k$ intervals, the value distribution after rescaling will match
the original unconditioned value distribution.  We refer to this transformation as \emph{extremal buffering}. We will show that applying this transformation approximately preserves the virtual surplus from each population in two steps. We first show that applying the transformation to one population in isolation does not significantly affect their expected virtual surplus. Second, we prove that applying the transformation to all other populations has a similarly small effect. Our analysis will hold for any choice of $k$. We will carefully select $k$ later.

We formally define and analyze the extremal buffering procedure in Section~\ref{sec:hedge}, and
the binning algorithm that results from resampling the buffered algorithm in
Section~\ref{sec:resample}. We will argue for an arbitrary monotone allocation algorithm, and a fairly general class of virtual value functions. Taking the allocation algorithm to be surplus maximization and the virtual value function to be value or Myerson virtual value will yield the following lemma:

\begin{lemma}\label{lem:binning}
		For each agent $i$, let $\phi_i(q_i)$ be a nonincreasing virtual value function, and let $\mathbf x$ be an a monotone allocation algorithm. There exists a surrogate binning algorithm with $T$ bins per population that treats the top $k$ and bottom $k$ bins identically for each population, and which obtains at least a $\frac{k}{k+1}(1-\frac{q}{1-q})(1-q)(1-2(n-1)q)$-fraction of the expected virtual surplus under $\mathbf x$, with $q=k/T$.
		%Further, for some $k\leq T/2$, let $\mathbf{\hat x}$ denote the $k/T$-buffering algorithm for $\mathbf x$. Then there exists a binning algorithm for $\mathbf{\hat x}$ obtains at least a $\frac{k}{k+1}(1-\frac{q}{1-q})(1-q)(1-2(n-1)q)$-fraction of the expected virtual surplus under $\mathbf x$, with $q=k/T$.
\end{lemma}

\subsubsection{Extremal Buffering}
\label{sec:hedge}
\label{SEC:HEDGE}

We have seen that na\"ively resampling each agent's value based on their bin cannot yield a mechanism with a good welfare or revenue approximation. We show now how to transform an arbitrary allocation algorithm to guarantee that not too much virtual surplus is lost from mishandling agents with extreme quantiles. The procedure follows:

\begin{definition}
	\label{def:hedge}
	Given a monotone allocation algorithm ${\mathbf x}$ and a quantile $q\in[0,1]$, the \emph{$q$-buffering algorithm} for
	${\mathbf x}$ runs ${\mathbf x}$ on agents with quantiles
	transformed for each agent as follows:
	\begin{itemize}
		\item For any $q_i\in[0,q]$, return 0.
		\item For any $q_i\in[q,1-q]$, return $(q_i-q)/(1-2q)$.
		\item For any $q_i\in [1-q,1]$, return $1$.
	\end{itemize}
\end{definition}

We will prove the following approximation guarantee:

\begin{lemma}
	\label{lem:toppromotion}
	\label{LEM:TOPPROMOTION}
	For each agent $i$, let $\phi_i:[0,1]\rightarrow \mathbb R$ be an arbitrary nonincreasing virtual value function satisfying $\int_0^1 \phi_i(q)\,dq\geq 0$. The $k/T$-buffering algorithm for $\mathbf{x}$ attains at least a $(1-\frac{q}{1-q})(1-q)(1-2(n-1)q)$-fraction
	of the virtual surplus of $\mathbf{x}$, with $q=k/T$.
\end{lemma}

The proof of Lemma~\ref{lem:toppromotion} will proceed in two main steps. First, we will show that applying the quantile remapping procedure in Definition~\ref{def:hedge} to a single population $i$ (leaving other populations' quantiles untouched) cannot reduce the expected virtual surplus from that population by too much. This will follow from a natural approximation result we derive, which relates the virtual surpluses of allocation rules with inverses that are multiplicatively close. Second, we will show that subsequently applying the quantile resampling procedure to the populations other than $i$ also does not significantly reduce the expected virtual surplus from $i$. This will follow from the fact that the distribution of quantiles input to the base allocation algorithm is identical, conditioned on no agents having extreme quantiles. 

We begin with the single-agent analysis. Note that for a single agent, the $q$-buffering procedure can be thought of as two composed steps. First is a \emph{top promotion} procedure, which remaps sufficiently low quantiles to $0$ while remapping the remaining quantiles to induce a uniform distribution over $[0,1]$. Top promotion is then composed with \emph{bottom demotion}, which performs analogous transformation, mapping high quantiles to $1$ and mapping the rest of the interval to $[0,1]$. We formalize this as follows:

\begin{definition}
	Given a monotone single-agent allocation rule $x$ and quantile $\underline q$, the \emph{top promotion algorithm} for $x$ and $\underline q$  runs $x$ on the agent with quantiles transformed as follows:
	\begin{itemize}
		\item For any $q\in[0,\underline q]$, return $0$.
		\item For any $q\in[\underline q,1]$, return $(q-\underline q)/(1-\underline q)$.
	\end{itemize}
\end{definition}

\begin{definition}
	Given a monotone single-agent allocation rule $x$ and quantile $\overline q$, the \emph{bottom demotion algorithm} for $x$ and $\overline q$ runs $x$ on the agent with quantiles transformed as follows:
	\begin{itemize}
		\item For any $q\in [0,\overline q]$, return $q/\overline q$.
		\item For any $q\in [\overline q, 1]$, return $1$.
	\end{itemize}
\end{definition}

The interim allocation rule faced by an agent $i$ after applying the extremal buffering algorithm to just $i$ is the composition of the bottom demotion algorithm for quantile $1-q$ composed with the top promotion algorithm for original allocation rule $x_i$ and quantile $q/1-q$.
Consequently, we may analyze the loss from applying these two transformations separately and multiply the losses.

We first analyze bottom demotion. While bottom demotion does not
produce an allocation rule which is multiplicatively close to the
original rule, it does produce one which is close in the sense that
its inverse is close to the inverse of the original rule. We may therefore apply  \Cref{lem:apx}
from \Cref{sec:BAR} which we restate here for convenience.  Recall, a virtual value
function is $\virt(\cdot)$ and has cumulative virtual curve
$\cumvirt(\quant) = \int_0^\quant \virt(r)\,dr$.

\begin{numberedlemma}{\ref{lem:apx}}
For virtual value function $\virt(\cdot)$ and cumulative virtual value
$\cumvirt(q)=\int_0^{\quant} \virt(r)\,dr$ satisfying $\cumvirt(\alpha
\,\quant)\geq \alpha\, \cumvirt(\quant)$ for all quantiles $\quant$
and $\alpha \in [0,1]$, and any two allocation rules $\alloc_1$ and
$\alloc_2$ that satisfy $\alloc_1^{-1}(z)\geq \alloc_2^{-1}(z)\geq
\tfrac{1}{\alpha}\alloc_1^{-1}(z)$, the virtual surpluses satisfy
	\begin{align*}
	\expect[\quant]{\virt(\quant)\,\alloc_2(\quant)} + \cumvirt(0)\,\alloc_2(0)
   &\geq \tfrac{1}{\alpha} [\expect[\quant]{\virt(\quant)\,\alloc_1(\quant)} + \cumvirt(0)\,\alloc_1(0). 
	\end{align*} 
\end{numberedlemma}


\begin{lemma}\label{lem:bottomdemote}
	Let $\phi:[0,1]\rightarrow\mathbb R$ be an arbitrary nonincreasing virtual value function. Given a monotone single-agent allocation rule x and quantile $\overline q$, the bottom demotion algorithm for $x$ and $\overline q$ obtains at least a $\overline q$-fraction of the expected virtual surplus of $x$.
\end{lemma}
\begin{proof}
	The lemma will follow from a straightforward application of Lemma~\ref{lem:apx}. For a quantile $q$ receiving allocation $x(q)$ from the base algorithm, the quantile receiving this probability of allocation under the bottom demotion algorithm will be $\overline q q$. Hence, $x^{-1}(z)\geq \hat x^{-1}(z)=\overline q x^{-1}(z)$. Since $\phi$ is nonincreasing in $q$, we have that $R(q)=\int_0^q \phi(r)\,dr$ satisfies $R(\alpha q)\geq \alpha R(q)$ for all $\alpha\in [0,1]$. Lemma~\ref{lem:apx} therefore implies the desired result.
\end{proof}

We have shown that bottom demotion results in an allocation rule which has an inverse close to that of the original rule on which it is based. To derive an approximation result for the top promotion algorithm requires 
 a more nuanced version of the same approach, based on two observations.
First, the ``unallocation rules'', i.e., $y(q) = 1-x(1-q)$ for allocation
rule $x(q)$, satisfy the inverse-approximation condition of the lemma.
Second, the virtual surplus of the unallocation rule is given by the
expected virtual value plus the negative virtual surplus of the
unallocation rule.  Specifically ${\mathbb E}_q[\phi(q)\,x(q)] =
{\mathbb E}_q[\phi(q)] + {\mathbb E}_q[(-\phi(1-q))\,y(q)]$.
While virtual values for revenue always satisfy the property that rays
from the origin cross the cumulative virtual value curve from below,
this property does not generally hold for the negative virtual values
$-\phi(1-q)$.  Regularity, i.e., monotonicity of the original virtual
value function, however, implies the property for negative virtual
values.  These observations are formally summarized in the subsequent
lemma:

\begin{lemma}\label{lem:toppromote}
	Let $\phi:[0,1]\rightarrow \mathbb R$ be a nonincreasing virtual value function with $\int_0^1 \phi(q)\,dq\geq 0$. Given a monotone single-agent allocation rule $x$ and quantile $\underline q$, the top promotion algorithm for $x$ and $\underline q$ obtains at least a $(1-\underline q)$-fraction of the expected virtual surplus of $x$.
\end{lemma}
\begin{proof}
Note that the expected virtual surplus from any allocation rule $x$ is can be written as $\int_0^1 \phi(q)x(q)\, d q=\int_0^1 \phi(q)\,dq-\int_0^1\phi(q)(1-x(q))\,dq$. Specifically, let $\hat x$ be the allocation rule of the top promotion algorithm, and $x$ the allocation rule of the original algorithm. Moreover, define $\hat y(q)=1-\hat x(1-q)$ and $y(q)=1-x(1-q)$ to be the corresponding ``unallocation rules.'' We will show that 
	\begin{equation}
	\label{eq:dealloc}
	\int_0^1-\phi(1-q)\hat y(q)\,dq \geq (1-\underline q) \int_0^1-\phi(1-q)y(q)\,dq.
	\end{equation}
	Since, $\int_0^1 \phi(q)\,dq\geq 0$, this will prove that $\int_0^1 \phi(q)x(q)\, d q\geq (1-\underline q)\int_0^1 \phi(q)\hat x(q)\, d q$.
	
	To prove (\ref{eq:dealloc}), note that the definition of the top promotion algorithm can be manipulated to obtain $\hat x^{-1}(z)=x^{-1}(z)(1-\underline q)+\underline q$. Moreover, by the definition of $y$ and $\hat y$, we have $y^{-1}=1-x^{-1}(1-z)$ and $\hat y^{-1}=1-\hat x^{-1}(1-z)$. Combining these three equations yields that $y^{-1}(z)\geq \hat y^{-1}(z)= (1-\underline q) y^{-1}(z)$ for all $z\in[0,1]$. Moreover, note that $-\phi(1-q)$ is decreasing in $q$. This implies that $R(q)/q\geq -\phi(1-q)$, where $R(q)=\int_0^q -\phi(1-q)\,dq$. We may therefore apply Lemma~\ref{lem:apx}, which yields (\ref{eq:dealloc}).
\end{proof}

Combining Lemmas~\ref{lem:bottomdemote} and~\ref{lem:toppromote} yields the following:
\begin{lemma}\label{lem:singleagent}
	Let $\phi:[0,1]\rightarrow \mathbb R$ be an arbitrary nonincreasing virtual value function satisfying $\int_0^1 \phi(q)\,dq\geq 0$, and consider an arbitrary agent $i$. The $q$-buffering algorithm for ${\mathbf x}$ and $\hat Q$, when applied only to agent $i$, attains at least a $(1-\frac{q}{1-q})(1-q)$-fraction of the expected virtual surplus for $i$.
\end{lemma}


Having derived a single-agent guarantee, we now show that applying the $q$-buffering algorithm to all agents at once, rather than just to one agent, yields only a small additional loss. Intuitively, for each agent, the mechanism only appears different when another agent has an extreme quantile which is promoted or demoted by the buffering algorithm. The probability of such an event can be bounded using the union bound. Formally, we have:

\begin{proof}[Proof of Lemma~\ref{lem:toppromotion}]
	
	Lemma~\ref{lem:singleagent} states that the virtual surplus lost from applying the $q$-buffering procedure to a single agent is small. We now argue that applying the algorithm to all agents at once does not incur much additional loss. We argue from the perspective of some agent $i$. 
	
	The key observation in our analysis is
	that the distribution of the quantiles of other agents is nearly unchanged by the extremal buffering algorithm.  In particular, note
	that the probability that one or more agents other
	than $i$ with quantiles set to $0$ or $1$ by the extremal buffering algorithm is at
	most $(n-1)(1-2q)$, by the union bound.  Conditioned on there being no
	such agents, the distribution of quantiles input to the allocation algorithm remains uniform. It follows that the virtual surplus from distribution $i$
	conditioned on this event is identical to the revenue from
	the extremal buffering algorithm applied only to $i$.
	
	In the event that there are one
	or more agents from populations other than $i$ who have top quantiles (which are promoted) or bottom quantiles (which are demoted), we note that the conditional virtual surplus from population $i$ is nonnegative. To see this, let $\tilde x_i$ be the interim allocation rule for agent $i$ in the $q$-buffering algorithm conditioned on the event $\mathcal E$ that at least one agent $j$ other than $i$ has a quantile in $[0,q]\cup[1-q,1]$. Since $\mathbf x$ is a monotone function of its inputs, it must be that $\tilde x_i$ is  nondecreasing. The expected virtual surplus from agent $i$ conditioned on $\mathcal E$ is $\int_0^1 \phi_i(q)\tilde x_i(q)\,dq$. By assumption, $\int_0^1 \phi_i(q)\,dq\geq 0$, so it must also be the case that $\int_0^1 \phi_i(q)\tilde x_i(q)\,dq\geq 0$.
	
	To conclude the proof, let $\hat x_i$ denote the interim allocation rule of the extremal buffering algorithm conditioned on the event $\overline{\mathcal E}$. The total virtual surplus from agent $i$ is:
	\begin{equation}
	\notag
	\text{Pr}(\mathcal E)\int_0^1 \phi_i(q)\tilde x_i(q)\,dq+\text{Pr}(\overline{\mathcal E})\int_0^1 \phi_i(q)\hat  x_i(q)\,dq
	\end{equation}
	By the union bound, $\text{Pr}(\overline{\mathcal E})=1-\text{Pr}(\mathcal E)\geq 1-(n-1)(1-2q).$ By Lemma~\ref{lem:singleagent} and the fact that, conditioned on $\overline{\mathcal E}$, the distribution of quantiles $i$ perceives from other agents is uniform implies that 
	\begin{eqnarray}
	\notag \int_0^1 \phi_i(q)\hat x_i(q)\,dq&\geq (1-\frac{q}{1-q})(1-q)\int_0^1 \phi_i(q)x_i(q)\,dq\\
	\notag &\geq (1-\frac{q}{1-q})(1-q)\int_0^1 \phi_i(q)x_i(q)\,dq.
	\end{eqnarray}
	Since we have shown that $\int_0^1 \phi_i(q)\hat  x_i(q)\,dq\geq 0$, we can combine the above to obtain:
	\begin{eqnarray}
	\notag
	\text{Pr}(\mathcal E)\int_0^1 \phi_i(q)\tilde x_i(q)\,dq+\text{Pr}(\overline{\mathcal E})\int_0^1 \phi_i(q)\hat  x_i(q)\,dq\\
	\notag \geq \big(1-\frac{q}{1-q}\big)(1-q)(1-2(n-1)q)\int_0^1\phi_i(q)x_i(q)\,dq.
	\end{eqnarray}
	Summing over agents proves the lemma.
\end{proof}

Since we have reasoned about abstract virtual surplus, which could be value or Myerson virtual value, we obtain revenue and welfare approximation results for the extremal buffering algorithm.

% \begin{corollary}
% 	Given a monotone allocation rule $\mathbf x$, and positive integer $k$, the $k/T$-quantile extremal buffering algorithm for $\mathbf x$ and $\hat Q$ obtains at least a $(1-\frac{q}{1-q})(1-q)(1-2(n-1)q)$-fraction of the expected welfare of $\mathbf x$. If agents' distributions are regular, then the $k$-bin extremal buffering algorithm obtains at least a $(1-\frac{q}{1-q})(1-q)(1-2(n-1)q)$-fraction of the revenue of $\mathbf x$ as well.
% \end{corollary}

\subsubsection{Approximately Optimal Resampling}
\label{sec:resample}

We previously observed that na\"ively resampling each agent's quantile from their bin could drastically reduce the welfare or revenue of an algorithm. Driving this loss were agents with extreme quantiles: if the base algorithm's welfare was driven primarily by allocating rare but high-valued agents while rejecting all other quantiles, it is very unlikely that the resampling procedure will give these high-valued agents priority.

Applying the $k/T$-buffering procedure for some $k$ before resampling solves exactly this issue. After applying the $k/T$-buffering procedure, resampling does not change the way the mechanism treats the top $k$ and bottom $k$ bins, as agents in those bins are already treated identically. Consequently, any loss from resampling must occur in the central quantiles of the distribution. For decreasing virtual value functions, such loss cannot be too high. In what follows, we formally define our resampling procedure, and then prove its performance guarantee.

% \begin{definition}
% \label{d:SBA}
% A {\em surrogate binning algorithm} is
% parameterized by $nT$ surrogate values, denoted $\Psi_i =
% \{\psi_i^1\geq\ldots\geq\psi_i^T\}$ for each agent $i$, and a allocation algorithm $\mathbf{x}$.  The mechansim takes as input a bid for every agent $i$. Given these inputs the surrogate binning algorithm assigns surrogate values $(\psi_1,\ldots, \psi_n)$ according to the binning selection rule for each agent's true distribution and outputs the allocation $\mathbf{\hat x}(\psi_1,\ldots, \psi_n)$.
% \end{definition}

\begin{definition}
	The \emph{resampling algorithm} for allocation algorithm $\mathbf{x}$ allocates according to the following randomized procedure:
\begin{itemize}
	\item For each agent $i$:
    \begin{itemize}
    	\item Compute $j$ such that $i$'s quantile $q_i\in[(j-1)/T,j/T]$.
        \item Resample a quantile uniformly from $[(j-1)/T,j/T]$.
 	\end{itemize}
 
  \item Runs $\mathbf x$ on the resampled quantiles.
\end{itemize}
\end{definition}

\begin{lemma}\label{lem:resampling}
		For each agent $i$, let $\phi_i(q_i)$ be a nonincreasing virtual value function, and let $\mathbf x$ be an a monotone allocation algorithm. Further, for some $k\leq T/2$, let $\mathbf{\hat x}$ denote the $k/T$-buffering algorithm for $\mathbf x$. Then the resampling algorithm for $\mathbf{\hat x}$ obtains at least a $\frac{k}{k+1}(1-\frac{q}{1-q})(1-q)(1-2(n-1)q)$ the expected virtual surplus under $\mathbf x$, with $q=k/T$.
\end{lemma}

Since the resampling algorithm is a surrogate binning mechanism, \Cref{lem:binning} immediately follows. To prove Lemma~\ref{lem:resampling}, we first rephrase a useful lemma from \citet{RS16}, which characterizes the relationship between the virtual surplus of resampling algorithms and their base algorithms. Informally, the result states that the revenue from bin-based resampling for an allocation rule $\mathbf x$ is the same as if $\mathbf x$ was run on the binned revenue curve for those same bins. Formally:

\begin{lemma}[\citealp{RS16}]\label{lem:switching}
	For every agent $i$, let $\phi_i$ be a virtual value function for each agent, with cumulative virtual surplus $R_i(q)=\int_0^q\phi_i(r)\,dr$. For any allocation algorithm $\mathbf x$, let $\mathbf{\overline x}$ denote the resampling algorithm based on $\mathbf x$. Then for each agent $i$ we have:
	\begin{equation}
	\mathbb E[-\overline x_i'(q_i)R_i(q_i)]=\mathbb E[-\overline x_i'(q_i)\overline R_i(q_i)]=\mathbb E[- x_i'(q_i)\overline R_i(q_i)],
	\notag
	\end{equation}
where $\overline R_i(q_i)$ is a piecewise linear approximation to $R_i$ given by:
\begin{equation}
\notag
\overline R_i(q)=T(q-\tfrac{j-1}{T})R_i(\tfrac{j}{T})+T(\tfrac{j}{T}-q)R_i(\tfrac{j-1}{T})\text{ for }q\in[\tfrac{j-1}{T},\tfrac{j}{T}].
\end{equation}
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lem:resampling}]
	Let $\mathbf{\hat x}$ denote the allocation rule of the $k/T$-buffering algorithm, and $\mathbf{\overline x}$ that of the resampling algorithm. Define
\begin{equation}
\notag
\hat R_i(q_i)=\begin{cases}
R_i(q_i)&\text{ for }q_i\in[\tfrac{k}{T},\tfrac{T-k}{T}]\\
\tfrac{Tq_i}{k}R_i(\tfrac{k}{T})&\text{ for }q_i\in[0,\tfrac{k}{T}]\\
R_i(\tfrac{T-k}{T})+\tfrac{T}{k}(q-\tfrac{T-k}{T})(R_i(1)-R_i(\tfrac{T-k}{T}))&\text{ for }q_i\in[\tfrac{T-k}{T},1].
%\tfrac{T(1-q_i)}{k}R_i(\tfrac{T-k}{T})&\text{ for }q_i\in[\tfrac{T-k}{T},1].\\
\end{cases}
\end{equation}
That is, $\hat R_i$ is equal to $R_i$ except on $[0,\tfrac{k}{T}]$ and $[\tfrac{T-k}{T},1]$, where it is a linear interpolation between the values of the $R_i$ at the endpoints of those intervals.
	
	We will argue the following sequence of inequalities for each agent:
	\begin{eqnarray}
	\notag\mathbb E[-\overline x_i'(q_i)R_i(q_i)]&=\mathbb E[-\hat x_i'(q_i)\overline R_i(q_i)]\\
	\notag&\geq \frac{k}{k+1}\mathbb E[-\hat x_i'(q_i)\hat R_i(q_i)]\\
	\notag&=\frac{k}{k+1}\mathbb E[-\hat x_i'(q_i)R_i(q_i)].
	\end{eqnarray}
	The first equality follows from Lemma~\ref{lem:switching}.
We will argue the second and third lines shortly.  Since the first and last expressions in the above chain are the respective virtual surpluses of the resampling and buffering algorithms, respectively, the result will follow.
	
	To see that $\overline R_i(q_i)\geq \tfrac{k}{k+1}\hat R_i(q_i)$, note that $\overline R_i(q_i)=\hat R_i(q_i)$ for all quantiles in $[0,\hat q_i^k]\cup[\hat q_i^{T-k},1]$. Otherwise, consider $q_i\in[\tfrac{j}{T},\tfrac{j+1}{T}]$ for $j\in\{k,\ldots,T-k-1\}$. Assume without loss of generality that $R_i(\tfrac{j}{T})\leq R_i(\tfrac{j+1}{T})$; a symmetric argument will apply to the case where $R_i(\tfrac{j}{T})\geq R_i(\tfrac{j+1}{T})$. The concavity of $R_i$ implies that for all $q\in[\tfrac{j}{T},\tfrac{j+1}{T}]$, $R_i(q)\leq \tfrac{Tq}{j}R_i(\tfrac{j}{T})$. Moreover, note that $\overline R_i(q)\geq R_i(\tfrac{j}{T})$ for all $q\in[\tfrac{j}{T},\tfrac{j+1}{T}]$. Since $\tfrac{Tq}{j}\leq \tfrac{k+1}{k}$, it follows that $\overline R_i(q_i)\geq \tfrac{k}{k+1} R_i(q_i)=\tfrac{k}{k+1}\hat R_i(q_i)$ for all $q_i\in[\tfrac{k}{T},\tfrac{T-k}{T}]$, and $\overline R_i(q_i)=\hat R_i(q_i)$ elsewhere.
    
    Finally, we argue that $\mathbb E[-\hat x_i'(q_i)\hat R_i(q_i)]=E[-\hat x_i'(q_i)R_i(q_i)]$. Note that since $\hat R_i(q_i)=R_i(q_i)$ for $q_i\in [\tfrac{k}{T},\tfrac{T-k}{T}]$, it follows that 
\begin{equation*}
    \int_{\tfrac{k}{T}}^{\tfrac{T-k}{T}} -\hat x_i(q_i)R_i(q_i)\, dq_i=\int_{\tfrac{k}{T}}^{\tfrac{T-k}{T}} -\hat x_i(q_i)\hat R_i(q_i)\, dq_i.
\end{equation*}
To prove the claim, notice that $\hat x_i'(q_i)=0$ on $[0,\tfrac{k}{T}]$ and $[\tfrac{T-k}{T},1]$. Hence,
\begin{equation*}
    \int_{0}^{\tfrac{k}{T}} -\hat x_i'(q_i)R_i(q_i)\, dq_i=\int_{0}^{\tfrac{k}{T}} -\hat x_i'(q_i)\hat R_i(q_i)\, dq_i.
\end{equation*}
and
\begin{equation*}
    \int_{\tfrac{T-k}{T}}^{1} -\hat x_i'(q_i)R_i(q_i)\, dq_i=\int_{\tfrac{T-k}{T}}^{1} -\hat x_i'(q_i)\hat R_i(q_i)\, dq_i.
\end{equation*}
This proves the lemma.
\end{proof}

% \begin{proof}[Proof of Theorem~\ref{thm:general}]
% We proved in Theorem~\ref{thm:binopt} that the mechanism which maximizes revenue for the binned revenue curves $R_i^{\hat Q}$ is optimal among all mechanisms which treat agents based only on their bin. It therefore inherits the revenue guarantees of the $k$-bin resampling mechanism for any choice of $k$. Choosing $k=\sqrt{n/T}$ and applying the bound of Lemma~\ref{lem:resampling} yields the result.
% \end{proof}
%We now define a surrogate-binning algorithm which retains all but a
%vanishing fraction of the surplus of $\mathbf{\hat x}$. To do so, we
%must choose a stage allocation algorithm, as well as a surrogate value
%for each interval in quantile space for each distribution. Our binning
%algorithm will use the top promotion algorithm from
%Section~\ref{sec:hedge} based on $\mathbf{\hat x}$ as its stage
%allocation algorithm. Our surrogate values will be chosen by random
%resampling. Formally:
%
%\begin{definition}
%The \emph{resampling algorithm} for allocation algorithm $\mathbf{\hat
%  x}$ is the surrogate binning mechanism whose stage algorithm is the
%top promotion algorithm for $\mathbf{\hat x}$ and with surrogate
%values given by:
%\begin{itemize}
%\item for $j\in \{1,\ldots,T-k\}$, determine $\psi_i^j$ by randomly sampling from distribution $F_i$ conditioned on the interval $[(j-1)/T,j/T]$ in quantile space.
%\item determine $\{\psi_i^j\}_{j=T-k+1}^T$ jointly by sampling and sorting $k$ values from $F_i$ conditioned on the interval $[(T-k)/T,1]$ in quantile space.
%\end{itemize}
%\end{definition}
%
%\begin{lemma}
%\label{lem:resample}
%\label{LEM:RESAMPLE}
%For any monotone stage allocation algorithm $\mathbf{\hat x}$ and $k<
%T/2$, the resampling algorithm attains a
%$(1-k/T)^2(1-k(n-1)/T)$-fraction of the welfare of $\mathbf{\hat
%  x}$. For regular value distributions, this bound holds for virtual
%surplus as well.
%\end{lemma}
%
%The lemma follows from noting that the resampling algorithm's allocation rule is a piecewise-constant approximation to the allocation rule of the top promotion algorithm.
%We show that the revenue of this approximation is close by integrating by parts the virtual surplus of any allocation rule $x$, $\mathbb E_{q\sim U[0,1]}[x(q)\phi(q)]$, to obtain $\mathbb E_{q\sim U[0,1]}[-X(q)\phi'(q)] + X(1)\phi(1)$, where $X(q)=\int_0^q x(s)\,ds$ is the cumulative allocation rule for $x$. Because the allocation rule for the resampling algorithm is a piecewise constant approximation to that of the top promotion algorithm, their cumulative allocation rules are multiplicatively close everywhere, which yields the result. The welfare result holds from identical reasoning.
%The full proof can be found in Appendix~\ref{APP:RESAMPLE}.
%

%\input{resampleapp}



\subsubsection{Proof of Theorem~\ref{thm:welfare}}

All that remains to prove the approximation result is to compose our lemmas and select a value for the parameter $k$. First, note the binning algorithm's surrogate values are the same for the intervals $[0,\tfrac{1}{T}],\ldots,[\tfrac{k-1}{T},\tfrac{k}{T}]$ and the intervals $[\tfrac{T-k}{T},\tfrac{T-k+1}{T}],\ldots,[\tfrac{T-1}{T},1]$. It follows that welfare and revenue loss from applying Theorem~\ref{thm:bvr} are both $O(k^{-1/2})$. Moreover, by \Cref{lem:resampling}, the resampling algorithm attains a $\frac{k}{k+1}(1-\frac{k/T}{1-k/T})(1-k/T)(1-2(n-1)k/T)$-fraction of the revenue and welfare of $\mathbf{\hat x}$. Composing these lemmas and setting $k=(n/T)^{2/3}$ yields the theorem.


==> inversesapp.tex <==
\section{Proof of Lemma~\ref{lem:apx}}
\label{app:inverses}

For any allocation rule $x(\cdot)$, we may write
\begin{equation}
\int_0^1\phi(q)x(q)\,dq=\int_0^1R(x^{-1}(z))dz.
\notag
\end{equation}
Now consider two arbitrary quantiles $q_1$ and $q_2$ satisfying $\tfrac{1}{\alpha}q_1\leq q_2\leq q_1$. By assumption, we have $R(q_2)\geq q_2R(q_1)/q_1\geq \tfrac{1}{\alpha}R(q_1)$. Since for all $z\in[0,1]$, we have assumed $\tilde x^{-1}(z)\geq \hat x^{-1}(z)\geq \tfrac{1}{\alpha}\tilde x^{-1}(z)$, this suffices to prove the lemma.

%We will prove the contrapositive to our claim: assume $R(q_2)< \tfrac{1}{\alpha}R(q_1)$. We will find a quantile $q^*$ such that $R(q^*)/q^*< \phi(q^*)$. By the continuity of $R(\cdot)$, there exists some $q'$ minimizing $R(q)/q$ in $[q_2,q_1)$. Choose the largest such $q'$. Moreover, there exists a smallest $q''$ in $(q_2,q_1]$ satisfying $q^*R(q_1)/q_1=R(q^*)$. By these definitions, we must have $R(q')\leq R(q_2)<\tfrac{1}{\alpha}R(q_1)\leq\tfrac{q_2}{q_1}R(q_1)=\tfrac{q_2}{q''}R(q'')\leq \tfrac{q'}{q''}R(q'')$.

%We next claim that for all $q\in [q',q'')$, $R(q)/q<R(q'')/q''$. Since $R(q_2)<\tfrac{1}{\alpha}R(q_1)$ and $\tfrac{1}{\alpha}q_1\leq q_2$, it must be that $R(q_2)/q_2<R(q_1)/q_1=R(q'')/q''$. Moreover, $R(q)/q$ is continuous. It follows that if $R(q)/q>R(q'')/q''$ for some $q\in [q',q'')$, there would have to be a quantile $p\in [q',q)$ with $R(p)/p=R(q'')/q''$, contradicting the definition of $q''$.

%We may now apply the mean value theorem: there is some $q^*\in[q',q'']$ such that 
%$$\phi(q^*)=\frac{R(q'')-R(q')}{q''-q'}>\frac{R(q'')-\tfrac{q'}{q''}R(q'')}{q''- q'}=\frac{R(q'')}{q''}>\frac{R(q^*)}{q^*}.$$



% In particular, let $q^*$ be the smallest quantile greater than $q_2$ such that $q^*R(q_1)/q_1=R(q^*)$. Since $R(q_2)<\tfrac{1}{\alpha}R(q_1)$, we have $q_2<q^*$. Furthermore, by the continuity of $R(\cdot)$, it must be that for $q\in (q_2,q^*)$, $R(q)< qR(q_1)/q_1$.

%First, define the cumulative virtual value of a quantile $q$ to be $R(q)=\int_0^q \phi(q)$. If $\phi(\cdot)$ is Myerson virtual value, then this is exactly the revenue curve of the distribution. The ex ante expected virtual surplus from an agent in terms of the cumulative virtual value curve is $E_{v_i}[\phi_i(v_i)x_i(v_i)]=\int_0^1 R'(q)x(q)\,dq$. We now write:
%\begin{align*}
%\int_0^1 R'(q)x(q)\,dq&=-\int_0^1 R(q)x'(q)\,dq\\
%&=\int_1^0 R(q)x'(q)\,dq\\
%&=\int_0^1 R(x^{-1}(z))\,dz,
%\end{align*}
%where the first equality follows from integrating by parts and noting that $R(0)=R(1)=0$ yields $-\int_0^1 R(q)x'(q)\,dq$, and the third from substituting $q=x^{-1}(z)$. To prove the theorem, we will use the fact that $\phi(\cdot)$ is decreasing, i.e. concavity of $R(\cdot)$, show that $R(\hat x^{-1}(q))\geq \tfrac{1}{\alpha}R(\tilde x^{-1}(q))$ for all quantiles $q$.

%Consider two arbitrary quantiles, $q_1$ and $q_2$ satisfying $\tfrac{1}{\alpha}q_1\leq q_2\leq q_1$. We will show $R(q_2)\geq \tfrac{1}{\alpha}R(q_1)$. We break the analysis into two cases:
%\begin{enumerate}
%\item $R(q_2)\geq R(\tfrac{1}{\alpha}q_1)$. In this case, concavity implies that $R(\tfrac{1}{\alpha}q_1)\geq \tfrac{1}{\alpha}R(q_1)$, which yields the desired inequaility.
%\item $R(q_2)< R(\tfrac{1}{\alpha}q_1)$. In this case, by concavity, $R$ is decreasing on $[\tfrac{1}{\alpha}q_1,q_1]$, and hence $R(q_2)\geq R(q_1)>\tfrac{1}{\alpha}R(q_1)$.
%\end{enumerate}
%In either case, $R(q_2)\geq \tfrac{1}{\alpha}R(q_1)$. Noting that $\tfrac{1}{\alpha}\tilde x^{-1} (q)\leq \hat x^{-1} (q)\leq \tilde x^{-1} (q)$ by assumption pr$•$oves the lemma.

==> newintro.tex <==
This paper builds a theory for mechanism design and redesign for
markets like Internet advertising where many frequent, small
transactions are organized by a principal.  In these environments
bidders place bids in advance and, as goods become available, the bids
of the relevant bidders are entered into an auction to determine the
allocation of goods.  In practice these auctions are not revelation
mechanisms, which introduces challenges for reasoning about their
design and, when bid data is available, their redesign.  Our theory
focuses on a salient model from auction theory, specifically the
independent private value model and auctions with winner-pays-bid or
all-pay payment semantics.

In general, good mechanisms for complex environments like the ones we
will consider have complex equilibria, their optimization is not
robust, and they generally require large amounts of data to optimize.
Our goal is to identify a family of practical mechanisms that exhibit
three properties.  First, we would like equilibria in these mechanisms
to be simple.  Second, we would like the mechanisms to be easily
reoptimized from the bid data that the mechanism generates.
Mechanisms from such a family could be tuned as fundamentals of the
market evolve.  Third, we would like the performance of mechanisms in
the family to be near the optimal performance possible by any
mechanism (not necessarily within the family).  This last property
implies that there is only modest loss to the principal in requiring
the first two properties.

Much of the theory of mechanism design is developed via the {\em
  revelation principle} \citep{M81} which observes that existence of a
mechanism with good equilibrium implies the existence of one with a
good truthtelling equilibrium.  
%The understanding of what is
%achievable by mechanisms is facilitated by the revelation principle,
%in particular, because it is without loss to search only over
%mechanisms that possess a truthtelling equilibrium.  
While revelation mechanisms are sometimes simple and robust, they do
not tend to arise in practice in markets like the ones we study, and
attempting to derive the corresponding non-revelation mechanism
preserves neither simplicity nor robustness (see
Appendix~\ref{app:unrevelation}).  Moreover, data-driven methods for
the design of revelation mechanisms \citep[e.g.,][]{CR-14} cannot be
applied directly to non-revelation mechanism as the bid data in
non-revelation mechanisms is, by definition, not equal to the true
preferences of the bidders.

We study mechanism design in the \emph{iterated population model}.  In this
model there are a collection of populations, and each population consists
of a continuum of bidders which induces a distribution of values.  The
strategies of these bidders induce a distribution of bids.  In each
iteration, one bidder from each population is drawn independently and
uniformly at random to participate in a mechanism. For example, the
mechanism might be the first price auction where the highest bidder
wins and pays her bid.  Notice that a single stage of this iterated
population model is equivalent to the standard independent private
value model that is pervasive in auction theory.  Our model simply is
an explicit extension of this standard model to an iterated
environment.


Our search for a simple family of mechanisms that satisfies the three
desiderata discussed above yields the following conclusions.  First,
while the classical theory tends to design and analyze mechanisms for
the stage environment, ignoring our assumption that the auction is
iterated over many stages, there is an advantage to linking the
decisions that are made across the stages.\footnote{A similar
observation was made by \citet{JS07} in the case where each agent is
returning repeatedly to the mechanism.  Our conclusion is conceptually
different from theirs as the decisions we are linking are between
distinct bidders from the same population.}  Second, the family of
mechanisms that we identify are {\em rank-based}, i.e., based only on
the order of bids from bidders in the same population and not the
cardinal values of the bids.  Thus, mechanisms in this family look, to
each population of bidders, like the i.i.d.\@ position auctions that
\citet{CH13} prove have simple, unique, and efficient equilibria.  Third, in
relation to data-driven methods in mechanism design, our approach uses
samples from the bid distribution in two distinct ways: (a) the family
of mechanisms is parameterized and these parameters can be optimized
from bid data using the simple and statistically efficient methods for
counterfactual estimation developed by \citet{CHN14}, cf.\@ the
literature on sample complexity in mechanism design; and (b) samples
from the bid distribution are used within the execution of the
mechanism to calculate the ranks of bidders (from which the mechanism
determines its outcome), cf.\@ the literature on prior-independent
mechanism design.

The second observation above, that the equilibria for each population
looks like an i.i.d.\@ position auction which only admits the
efficient equilibrium, gives us a ``revelation principle'' for
non-revelation mechanisms.  The efficient equilibrium assigns bidders
to positions in the same order as their values.  Thus, the outcome
(and, e.g., welfare) of the mechanism is the same as it would be if
the bidders reported their values (even though doing so is not an
equilibrium).  Consequently, our approach gives the benefits of
revelation mechanism design, namely that analysis is straightforward
from bidder values, but for simple and practical mechanisms that do
not have truthtelling as an equilibrium.

Our analysis is based on several natural new approximation results
that compare pricing and ranking mechanisms.  This analysis is
reminiscent of the correlation gap work of \citet{Y11} and may be of
independent interest.


==> oldapproximation.tex <==
\section{Approximation Analysis}
\label{sec:BAR}
%TODO: switch n to T in bin vs rank analysis.

In this section, we state and briefly discuss our approximation
analysis for surrogate ranking mechanisms. Condition
\Cref{cond:performance} requires that there exist some choice of
surrogate values which induces near-optimal expected performance. 
%In \Cref{app:approximation},
In the full version of the paper,
we show how to construct a choice of
surrogate values which proves the following guarantee:
\begin{theorem}
\label{thm:welfare}
\label{THM:WELARE}
There exists a surrogate-ranking mechanism with winner-pays-bid, all-pay, or
truthful payment semantics which attains a $(1-
O(\sqrt[3]{n/\num}))$-fraction of the optimal welfare in stationary equilibrium. With regular distributions, there exists such a mechanism which attains a $(1-
O(\sqrt[3]{n/\num}))$-fraction of the optimal revenue in stationary
equilibrium.
\end{theorem}

\Cref{THM:WELARE} implies that the representation error of SRMs is low. In \Cref{sec:inference}, we show how to estimate a SRM which is nearly welfare- or revenue-optimal among all mechanisms in the family. This mechanism consequently inherits the guarantees of \Cref{THM:WELARE}, up to error from estimation.

The proof of \Cref{thm:welfare} is technically involved, and we defer details to the full verison of the paper. The high
level approach involves two main steps. We first argue that there exists an
approximately-optimal mechanism which coarsens quantile space into
bins, and treats agents based solely on their bin. We then show that
this bin-based mechanism can be transformed into a surrogate-ranking
mechanism with only polynomial loss in performance. 

A main challenge in proving approximation bounds in sample complexity
is arguing that agents at the extremes, i.e., quantiles close to 0 and
1, are treated appropriately.  For revenue, allocation to quantiles
close to 0 could have high positive contribution to the revenue while
allocation to quantiles close to 1 could have high negative
contribution to the revenue.  Our approach is to treat all agents that
have quantile close to 0 as if they have quantile 0 and all who have
quantile close to 1 as if they have quantile 1.  The key step in the
analysis is then to show that the loss from this change, which
disrupts the allocation to other agents, is bounded.  The subsequent
analysis is then relatively straightforward.

A key lemma in the analysis bounds virtual surplus from
allocation rules that are approximately similar and may be of
independent interest.  Recall the characterization of expected revenue
in terms of revenue curves and marginal revenue from \Cref{lem:vvals}:
\begin{align}
\label{eq:virtualsurplus}
\sexpect[\quant]{\price(\quant)} 
&= 
\sexpect[\quant]{-\alloc'(\quant)\,\rev(\quant)} + \rev(1)\,\alloc(1)
= 
\sexpect[\quant]{\marg(\quant)\,\alloc(\quant)} + \rev(0)\,\alloc(0).
\end{align} 
The first equality enables a geometric understanding of revenue.
Given an fixed allocation rule $\alloc$ in quantile
space, for two value functions $\vali[1]$ and $\vali[2]$ where
$\revi(\quant) = \quant\,\vali(\quant)$ satisfies $\revi[1](\quant)
\geq \revi[2](\quant)$, then the revenue from $\vali[1]$ on $\alloc$
is at least the revenue of $\vali[2]$ on $\alloc$.  This follows from
the first equality of equation \eqref{eq:virtualsurplus}, where the
expressions for revenue of both value functions are weighted integrals
over $\quant\in[0,1]$ with non-negative weights $-\alloci'(\quant)$.
Approximation bounds hold as well, specifically, if $\revi[2]$
approximates $\revi[1]$ at all $\quant\in[0,1]$ then the same
approximation holds for the revenue of any fixed allocation rule
$\alloc$. Note however that a similar result, with a fixed distribution and similar allocation rules is not implied by the second equation, as
the weights $\marg(\quant)$ are not generally all the same sign.  Instead, the
following lemma 
%considers the approximation of the inverse allocation
%rule and 
shows that two allocation rules with \emph{inverses} that are
approximately close have approximately the same revenue.  We state the
result for general virtual value functions $\virt(\cdot)$ and
cumulative virtual curves $\cumvirt(\quant) = \int_0^\quant
\virt(r)\,dr$.  The assumption in the lemma on the cumulative virtual
curve is that lines from the origin pass from below to above the
curve.  This assumption, for example, is satisfied by any revenue
curve, specifically, it does not require regularity.


\begin{lemma}
\label{lem:apx}
For virtual value function $\virt(\cdot)$ and cumulative virtual value
$\cumvirt(q)=\int_0^{\quant} \virt(r)\,dr$ satisfying $\cumvirt(\alpha
\,\quant)\geq \alpha\, \cumvirt(\quant)$ for all quantiles $\quant$
and $\alpha \in [0,1]$, and any two allocation rules $\alloc_1$ and
$\alloc_2$ that satisfy $\alloc_1^{-1}(z)\geq \alloc_2^{-1}(z)\geq
\tfrac{1}{\alpha}\alloc_1^{-1}(z)$, the expected virtual surpluses satisfy
	\begin{align*}
	\expect[\quant]{\virt(\quant)\,\alloc_2(\quant)} + \cumvirt(0)\,\alloc_2(0)
   &\geq \tfrac{1}{\alpha} [\expect[\quant]{\virt(\quant)\,\alloc_1(\quant)} + \cumvirt(0)\,\alloc_1(0)]. 
	\end{align*} 
\end{lemma}

\begin{proof}
The virtual surplus of any allocation rule $\alloc$ can be rewritten
as $\int_0^1\virt(\quant)\,\alloc(q)\,dq + \cumvirt(0)\,\alloc(0) =
\int_0^1 \cumvirt(\alloc^{-1}(z))\,dz$. This follows by the first
equality of equation \eqref{eq:virtualsurplus} and a change of
variables to integrate the vertical axis rather than the horizontal
axis as follows:
\begin{align}
\notag
\int_0^1 {-\alloc'(\quant)\,\cumvirt(\quant) \, d\quant} + \cumvirt(1)\,\alloc(1) 
	&= \int_{\alloc(1)}^{\alloc(0)} \cumvirt(x^{-1}(z))\, dz + \int_{0}^{\alloc(1)} \cumvirt(1)\, dz\\
\label{eq:inverse}
	&= \int_{0}^{\alloc(0)} \cumvirt(\alloc^{-1}(z))\, dz.
\end{align}
Notice that the second line follows from the first line because $\alloc^{-1}(z) = 1$ for $z \in [0,\alloc(1)]$.
	
Now consider two arbitrary quantiles $\quant_1$ and $\quant_2$
satisfying $\tfrac{1}{\alpha}\quant_1\leq \quant_2\leq \quant_1$. By
assumption, we have $\cumvirt(\quant_2)\geq
\quant_2\cumvirt(\quant_1)/\quant_1\geq
\tfrac{1}{\alpha}\cumvirt(\quant_1)$. The assumption on the
approximation of the two allocation rules, namely $\alloc^{-1}(z)\geq
\ealloc^{-1}(z)\geq \tfrac{1}{\alpha}\alloc^{-1}(z)$ for all
$z\in[0,1]$, and the expected virtual surplus written as rewritten in
equation~\eqref{eq:inverse} both both $\alloc_1$ and $\alloc_2$, then,
suffice to prove the lemma.
\end{proof}

==> promotionapp.tex <==
\section{Proofs from Section~\ref{sec:hedge}}
\label{APP:PROMOTION}

\begin{proof}[Proof of Lemma~\ref{lem:apx}]
%The proof rewrites the expected virtual surplus in terms of the
%cumulative virtual value curve via an integration by parts.  From this
%restatement, and the assumption on cumulative virtual value curves,
%the lemma follows.
%
The virtual surplus can be rewritten as $\int_0^1\phi(q)x(q)\,dq = \int_0^1 R(x^{-1}(z))dz$. This follows from an integration by parts and then change of variables to integrate the vertical axis rather than the horizontal axis as follows:
\begin{align}
\int_0^1\phi(q)x(q)\,dq &= R(1)x(1) - R(0)x(0) + \int_0^1 R(q)\, (-x'(q))\, dq\\\notag 
                        &= \int_0^{x(1)} R(1)\, dz - 0 + \int_{x(1)}^1 R(x^{-1}(z))\, dz.
\end{align}



Now consider two arbitrary quantiles $q_1$ and $q_2$ satisfying
$\tfrac{1}{\alpha}q_1\leq q_2\leq q_1$. By assumption, we have
$R(q_2)\geq q_2R(q_1)/q_1\geq \tfrac{1}{\alpha}R(q_1)$. The assumption
on the approximation of the two allocation rules, namely $\tilde
x^{-1}(z)\geq \hat x^{-1}(z)\geq \tfrac{1}{\alpha}\tilde x^{-1}(z)$
for all $z\in[0,1]$, and the expected virtual surplus written as $\int_0^1 R(x^{-1}(z))dz$ suffice to prove
the lemma.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:toppromotion}]
Consider the perspective of an agent $i$ in an arbitrary stage $t$. We
argue that their individual contribution to surplus cannot decrease by
more than a $k(n-1)/T$ fraction. This hinges on two key steps: we
first analyze the effect of the procedure when applied to just one
population $i$, and show that there is no loss to welfare, and at most
a $k/T$-fraction of revenue lost. We then analyze the effect on $i$'s
welfare and revenue when the procedure is applied to other
populations as well. Multiplying these approximation factors results in the total loss.

First, note that applying the top promotion algorithm to just
population $i$ only increases the probability that the agent is
allocated, as her promoted quantile is always lower than her original
quantile. Since values are always positive, this will only improve the
welfare contribution of distribution $i$.

Analysis of revenue is more complicated because virtual values may be
negative. Consequently, a stronger allocation rule need not improve
the revenue from population $i$.  We nonetheless can show that revenue
is not hurt by too much by applying Lemma~\ref{lem:apx} to the
``unallocation rule'' $y(q)=1-x(1-q)$. Note that $y(q)$ is decreasing
in $q$ and that $\int_0^1 \phi(1-q)\,y(q)\,dq$ is the total negative
virtual surplus left unallocated by $x$.

%and that for regular distributions, $\phi(q)$ is increasing with respect to $y(q)$. 

Formally, note that the expected revenue from any allocation rule $x$ is can be written as $\int_0^1 \phi(q)x(q)\, d q=\int_0^1 \phi(q)\,dq-\int_0^1\phi(q)(1-x(q))\,dq$. Specifically, let $x$ be the allocation rule of the top promotion algorithm, and $\hat x$ the allocation rule of the original stage algorithm. Moreover, define $y(q)=q-x(1-q)$ and $\hat y(q)=1-\hat x(1-q)$ to be the corresponding ``unallocation rules.'' We will show that 
\begin{equation}
\label{eq:dealloc}
\int_0^1-\phi(1-q)y(q)\,dq \geq \tfrac{k}{T}\int_0^1-\phi(1-q)\hat y(q)\,dq.
\end{equation}
Since as a basic fact about virtual values, $\int_0^1 \phi(q)\,dq\geq 0$, this will prove that $\int_0^1 \phi(q)x(q)\, d q\geq (1-\tfrac{k}{T})\int_0^1 \phi(q)\hat x(q)\, d q$.

To prove (\ref{eq:dealloc}), note that for any quantile $q$ receiving allocation $\hat x(q)$ from the stage algorithm, the quantile receiving this probability under the top promotion algorithm will be $1-\tfrac{k}{T}(1-q)$. It follows that $\hat y^{-1}(z)\geq y^{-1}(z)=\tfrac{k}{T}\hat y^{-1}(z)$ for all $z\in[0,1]$. Moreover, note that $-\phi(1-q)$ is decreasing in $q$. This implies that $R(q)/q\geq -\phi(1-q)$, where $R(q)=\int_0^q -\phi(1-q)\,dq$. We may therefore apply Lemma~\ref{lem:apx}, which yields (\ref{eq:dealloc}).



%First note that we can rearrange the integral formula for expected revenue as $\int_0^1 \phi(q)x(q)\, d r=\int_0^1 \int_{r:x(r)\geq z}\phi(r)\,dr\,dz$. Moreover, since the expected virtual value of any agent is nonnegative, we have $\int_0^1 \phi(r)\,dr\geq 0$. Consequently, the expected revenue is at least $-\int_0^1 \int_{r:x(r)< z}\phi(r)\,dr\,dz$.



%To prove that the remapping algorithm does not reduce the revenue by more than a $k/T$ factor, we will show that
%\begin{equation}
%\label{eq:tricky}
%\int_{r:y(r)\leq z}\phi(r)\,dr\leq (1-k/T)\int_{r:x(r)\leq z}\phi(r)\,dr,
%\end{equation}
%where $y(\cdot)$ is the allocation rule of the remapping algorithm.

%Consider some quantile $q$ such that $x(q)=z$. Under the remapping procedure, the quantile $q'$ with $y(q')=z$ will be $\hat q=1-\tfrac{k}{T}(1-q)>q$. It follows that for this $z$,
%\begin{align*}
%\int_{r:x(r)\leq z}\phi(r)\,dr-\int_{r:y(r)\leq z}\phi(r)\,dr&=\int_{q}^1\phi(r)%\,dr-\int_{\hat q}^1\phi(r)\,dr\\
%&=\int_q^{\hat q}\phi(r)\,dr
%\end{align*}

%Notice that $\hat q-q=\tfrac{k}{T}(1-q)$. Since $\phi(r)$ is nonincreasing in $r$, it follows that the virtual values which go uncounted in $\int_{r:y(r)\leq z}\phi(r)\,dr$, namely those between $q$ and $\hat q$, represent the highest $k/T$-fraction of virtual values from $[q,1]$. It follows that
%\begin{equation}
%\int_q^{\hat q}\phi(r)\,dr\geq \frac{k}{T}\int_{r:x(r)\leq z}\phi(r)\,dr,
%\notag
%\end{equation}
%which implies equation (\ref{eq:tricky}). We may now integrate equation (\ref{eq:tricky}) over all $z$ and multiply by $-1$ to produce the desired revenue bound.

We have shown that for both welfare and revenue, the top promotion
algorithm preserves a $(1-k/T)$-fraction (or better, for welfare) of
the objective of $x$ from a single population $i$, when applied to
only agents in $i$. We now analyze the effect on the welfare and
revenue of the agent from population $i$ from top promotion applied to
the $n-1$ other populations.  The key observation in our analysis is
that the distribution of the quantiles of agents from the other
population is nearly unchanged by top promotion.  In particular, note
that the probability that one or more agents from distributions other
than $i$ with quantiles set to 0 by the top promotion algorithm is at
most $(n-1)k/T$ by the union bound.  Conditioned on there being no
such agents, the distribution of quantiles from the top promotion
algorithm remains uniform.  It follows that the revenue and welfare
conditioned on this event is identical to the revenue from
$\mathbf{\hat x}$.  On the other hand, in the event that there is one
or more agents from populations other than $i$ who have top quantiles (which are promoted), the conditional welfare and virtual welfare is non-negative.

The (virtual) surplus from population $i$ from the top promotion
algorithm can be written as the approximation from promotion
population in $i$, i.e.\@ $(1-k/T)$, composed with the loss from
applying the procedure to all other agents, i.e.\@ $(1-k(n-1)/T)$. The
bound in the statement of the lemma results.
\end{proof}
